Calibrated Regression Against An Adversary Without Regret

We are interested in probabilistic prediction in online settings in which data does not follow a probability distribution. Our work seeks to achieve two goals: (1) producing valid probabilities that accurately reflect model confidence; and (2) ensuring that traditional notions of performance (e.g., high accuracy) still hold. We introduce online algorithms guaranteed to achieve these goals on arbitrary streams of data points, including data chosen by an adversary. Specifically, our algorithms produce forecasts that are (1) calibrated -- i.e., an 80% confidence interval contains the true outcome 80% of the time -- and (2) have low regret relative to a user-specified baseline model. We implement a post-hoc recalibration strategy that provably achieves these goals in regression; previous algorithms applied to classification or achieved (1) but not (2). In the context of Bayesian optimization, an online model-based decision-making task in which the data distribution shifts over time, our method yields accelerated convergence to improved optima.

==> checklist.tex <==
\section*{Checklist}


 \begin{enumerate}


 \item For all models and algorithms presented, check if you include:
 \begin{enumerate}
   \item A clear description of the mathematical setting, assumptions, algorithm, and/or model. [Yes]
   \item An analysis of the properties and complexity (time, space, sample size) of any algorithm. [Yes]
   \item (Optional) Anonymized source code, with specification of all dependencies, including external libraries. [No]
 \end{enumerate}


 \item For any theoretical claim, check if you include:
 \begin{enumerate}
   \item Statements of the full set of assumptions of all theoretical results. [Yes]
   \item Complete proofs of all theoretical results. [Yes]
   \item Clear explanations of any assumptions. [Yes]     
 \end{enumerate}


 \item For all figures and tables that present empirical results, check if you include:
 \begin{enumerate}
   \item The code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL). [Yes]
   \item All the training details (e.g., data splits, hyperparameters, how they were chosen). [Yes]
         \item A clear definition of the specific measure or statistics and error bars (e.g., with respect to the random seed after running experiments multiple times). [Yes]
         \item A description of the computing infrastructure used. (e.g., type of GPUs, internal cluster, or cloud provider). [Yes]
 \end{enumerate}

 \item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets, check if you include:
 \begin{enumerate}
   \item Citations of the creator If your work uses existing assets. [Yes]
   \item The license information of the assets, if applicable. [Not Applicable]
   \item New assets either in the supplemental material or as a URL, if applicable. [Not Applicable]
   \item Information about consent from data providers/curators. [Not Applicable]
   \item Discussion of sensible content if applicable, e.g., personally identifiable information or offensive content. [Not Applicable]
 \end{enumerate}

 \item If you used crowdsourcing or conducted research with human subjects, check if you include:
 \begin{enumerate}
   \item The full text of instructions given to participants and screenshots. [Not Applicable]
   \item Descriptions of potential participant risks, with links to Institutional Review Board (IRB) approvals if applicable. [Not Applicable]
   \item The estimated hourly wage paid to participants and the total amount spent on participant compensation. [Not Applicable]
 \end{enumerate}

 \end{enumerate}


==> figures/Makefile <==
LATEX = pdflatex
#LATEX = pdflatex -interaction=nonstopmode
FIGURES = $(wildcard *.tikz)
PDFS = $(patsubst %.tikz,%.pdf,$(FIGURES))

all:
	make synth.pdf
	make semparse.pdf
	make wtccc.pdf

# all: $(PDFS)

# %.pdf: %.tikz
# 	$(LATEX) $<

clean:
	rm -rf *.{aux,bbl,blg,log,out}
	rm -rf $(OUTPUT).pdf

.PHONY: clean bib final

semparse.pdf: data
	python ./calibration-plots.py \
	  --cal data/semparse-cal.txt \
	  --hist data/semparse-hist.txt \
	  --metrics data/semparse-metrics.txt \
	  --plots data/semparse-plots.txt \
	  --out $@

wtccc.pdf: data
	python ./calibration-plots.py \
	  --cal data/wtccc-cal.txt \
	  --hist data/wtccc-hist.txt \
	  --metrics data/wtccc-metrics.txt \
	  --plots data/wtccc-plots.txt \
	  --out $@

synth.pdf: data
	python ./synth-calibration-plots.py \
	  --bernoulli-plots ./data/synthetic-bernoulli.txt \
	  --adversarial-plots ./data/synthetic-adversarial.txt \
	  --out $@


==> figures/data/Makefile <==
SCRIPTS:=../scripts
DATA:=../data
TARGET:=../../doc/aistats2016/figures/data

all:
	make semparse
	make wtccc
	make synthetic-bernoulli.txt
	make synthetic-adversarial.txt
	make copy

copy:
	cp ./*.txt $(TARGET)

semparse:
	echo $(PYTHONPATH)
	python $(SCRIPTS)/gen-semparse.py \
	  --val $(DATA)/semparse/train.log \
	  --test $(DATA)/semparse/test.log \
	  --out-cal ./semparse-cal.txt \
	  --out-hist ./semparse-hist.txt \
	  --out-metrics ./semparse-metrics.txt \
	  --out-plots ./semparse-plots.txt
	touch $@

wtccc:
	python $(SCRIPTS)/gen-wtccc.py \
	  --cases $(DATA)/wtccc/T1D.top.sorted.input \
	  --controls $(DATA)/wtccc/58C.top.sorted.input \
	  --out-cal ./wtccc-cal.txt \
	  --out-hist ./wtccc-hist.txt \
	  --out-metrics ./wtccc-metrics.txt \
	  --out-plots ./wtccc-plots.txt
	touch $@

synthetic-bernoulli.txt:
	python $(SCRIPTS)/recalibration-bernoulli.py --out-plots $@

synthetic-adversarial.txt:
	python $(SCRIPTS)/recalibration-adversarial.py --out-plots $@

